Low-level Online Control of the Formula 1 Power Unit with Feedforward Cylinder Deactivation

Since 2014, the F\'ed\'eration Internationale de l'Automobile has prescribed a parallel hybrid powertrain for the Formula 1 race cars. The complex low-level interactions between the thermal and the electrical part represent a non-trivial and challenging system to be controlled online. We present a novel controller architecture composed of a supervisory controller for the energy management, a feedforward cylinder deactivation controller, and a track region-dependent low-level nonlinear model predictive controller to optimize the engine actuators. Except for the nonlinear model predictive controller, the proposed controller subsystems are computationally inexpensive and are real time capable. The framework is tested and validated in a simulation environment for several realistic scenarios disturbed by driver actions or grip conditions on the track. In particular, we analyze how the control architecture deals with an unexpected gearshift trajectory during an acceleration phase. Further, we demonstrate how an increased maximum velocity trajectory impacts the online low-level controller. Our results show a suboptimality over an entire lap with respect to the benchmark solution of 49 ms and 64 ms, respectively, which we deem acceptable. Compared to the same control architecture with full knowledge of the disturbances, the suboptimality amounted to only 2 ms and 17 ms. For all case studies we show that the cylinder deactivation capability decreases the suboptimality by 7 to 8 ms.

==> pictures/engineGearbox.tex <==
\makeatletter
%

\newcommand{\disPistone}{ %
	\pgfpathlineto{\pgfpointadd{\pgfpoint{\pgf@x}{\pgf@y}}{\pgfqpoint{0pt}{\pistoneh}}}
		\pgfpathlineto{\pgfpointadd{\pgfpoint{\pgf@x}{\pgf@y}}{\pgfqpoint{-\pistoneww}{0pt}}}
		\pgfpathlineto{\pgfpointadd{\pgfpoint{\pgf@x}{\pgf@y}}{\pgfqpoint{\pistonew}{0pt}}}
	\pgfpathmoveto{\pgfpointadd{\pgfpoint{\pgf@x}{\pgf@y}}{\pgfqpoint{-\pistoneww}{-\pistoneh}}}
}

\pgfdeclareshape{engine}{
	\inheritsavedanchors[from=rectangle] %
	\inheritanchorborder[from=rectangle]
	\inheritanchor[from=rectangle]{center}
	\inheritanchor[from=rectangle]{north}
	\inheritanchor[from=rectangle]{south}
	\inheritanchor[from=rectangle]{west}
	\inheritanchor[from=rectangle]{east}
	\inheritanchor[from=rectangle]{north west}
	\inheritanchor[from=rectangle]{north east}
	\inheritanchor[from=rectangle]{south east}
	\inheritanchor[from=rectangle]{south west}

	%
	
%
%
%
%
%
%
%

	\anchor{shaft}{
		\pgfpointdiff{\southwest}{\northeast}
		\pgf@xa=\pgf@x		%
		\pgf@ya=\pgf@y
		\southwest
		\pgf@xc=\pgf@x		%
		\pgf@yc=\pgf@y		%
		\advance\pgf@xc by -.1\pgf@xa
		\advance\pgf@yc by .225\pgf@ya
		\pgf@x=\pgf@xc
		\pgf@y=\pgf@yc
	}
	
	
	\anchor{tank}
	{
		\pgfpointdiff{\southwest}{\northeast}
		\pgf@xa=\pgf@x		%
		\pgf@ya=\pgf@y
		\southwest
		\pgf@xc=\pgf@x		%
		\pgf@yc=\pgf@y		%
		\advance\pgf@yc by .225\pgf@ya
		\northeast
		\pgf@y=\pgf@yc
	}
	
	\foregroundpath{%
		%
		\southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
		\northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
		\pgfpointdiff{\southwest}{\northeast}
		\pgf@xc=\pgf@x		%
		\pgf@yc=\pgf@y		%
		
		
		\gdef\inset{0.1\pgf@yc}
		\gdef\outsetwt{.1\pgf@xc}
		\gdef\outsetht{.25\pgf@yc}
		\def\lunghbiella{.14\pgf@xc}
		\def\lunghbiellaa{.07\pgf@xc}
		\def\pistoneh{.2\pgf@yc}
		\def\pistonew{.14\pgf@xc}
		\def\pistoneww{.07\pgf@xc}
		\def\xshiftbeginning{-.04\pgf@xc}
		
		%
		\pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
		\pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@ya}}
		%
		\pgfpathlineto{\pgfpointadd{\northeast}{\pgfqpoint{0pt}{-\inset}}}
		\pgfpathlineto{\pgfpointadd{\northeast}{\pgfqpoint{-\inset}{-\inset}}}
		\pgfpathlineto{\pgfpointadd{\northeast}{\pgfqpoint{-\inset}{0pt}}}
		%
		\pgfpathlineto{\pgfpointadd{\pgfpoint{\pgf@xa}{\pgf@yb}}{\pgfqpoint{\inset}{0pt}}}
		\pgfpathlineto{\pgfpointadd{\pgfpoint{\pgf@x}{\pgf@y}}{\pgfqpoint{0pt}{-\inset}}}
		\pgfpathlineto{\pgfpointadd{\pgfpoint{\pgf@x}{\pgf@y}}{\pgfqpoint{-\inset}{0pt}}}
		%
		\pgfpathlineto{\pgfpointadd{\pgfpoint{\pgf@x}{\pgf@y}}{\pgfqpoint{0pt}{-.55\pgf@xc}}}
		\pgfpathlineto{\pgfpointadd{\pgfpoint{\pgf@x}{\pgf@y}}{\pgfqpoint{-\outsetwt}{0pt}}}
		\pgfpathlineto{\pgfpointadd{\pgfpoint{\pgf@x}{\pgf@y}}{\pgfqpoint{0pt}{-\outsetht}}}
		\pgfpathlineto{\pgfpointadd{\pgfpoint{\pgf@x}{\pgf@y}}{\pgfqpoint{\outsetwt}{0pt}}}
		\pgfclosepath
		\pgfusepath{stroke}
		%
		%
		%
		%
		\pgfpathmoveto{\pgfpoint{\xshiftbeginning}{0pt}}
		\disPistone
		\pgfpathlineto{\pgfpointadd{\pgfpoint{\pgf@x}{\pgf@y}}{\pgfqpoint{-\lunghbiellaa}{0pt}}}
		\pgfpathlineto{\pgfpointadd{\pgfpoint{\pgf@x}{\pgf@y}}{\pgfqpoint{0pt}{-\lunghbiella}}}
		\pgfpathlineto{\pgfpointadd{\pgfpoint{\pgf@x}{\pgf@y}}{\pgfqpoint{-\lunghbiellaa}{0pt}}}
		%
		\disPistone
		\pgfpathlineto{\pgfpointadd{\pgfpoint{\pgf@x}{\pgf@y}}{\pgfqpoint{-\lunghbiellaa}{0pt}}}
		%
		\pgfpathlineto{\pgfpointadd{\pgfpoint{\pgf@x}{\pgf@y}}{\pgfqpoint{0pt}{\lunghbiella}}}
		\pgfpathlineto{\pgfpointadd{\pgfpoint{\pgf@x}{\pgf@y}}{\pgfqpoint{-\lunghbiellaa}{0pt}}}
		%
		\disPistone
		\pgfpathlineto{\pgfpointadd{\pgfpoint{\pgf@x}{\pgf@y}}{\pgfqpoint{-\lunghbiellaa}{0pt}}}
		\pgfpathlineto{\pgfpointadd{\pgfpoint{\pgf@x}{\pgf@y}}{\pgfqpoint{0pt}{-\lunghbiella}}}
		\pgfpathlineto{\pgfpointadd{\pgfpoint{\pgf@x}{\pgf@y}}{\pgfqpoint{-\lunghbiellaa}{0pt}}}
		%
		%
		%
		%
		\pgfpathmoveto{\pgfpoint{\xshiftbeginning}{0pt}}
		\pgfpathlineto{\pgfpointadd{\pgfpoint{\pgf@x}{\pgf@y}}{\pgfqpoint{\lunghbiellaa}{0pt}}}
		\pgfpathlineto{\pgfpointadd{\pgfpoint{\pgf@x}{\pgf@y}}{\pgfqpoint{0pt}{-\lunghbiella}}}
		\pgfpathlineto{\pgfpointadd{\pgfpoint{\pgf@x}{\pgf@y}}{\pgfqpoint{\lunghbiellaa}{0pt}}}
		\disPistone
		\pgfpathlineto{\pgfpointadd{\pgfpoint{\pgf@x}{\pgf@y}}{\pgfqpoint{\lunghbiellaa}{0pt}}}
		\pgfpathlineto{\pgfpointadd{\pgfpoint{\pgf@x}{\pgf@y}}{\pgfqpoint{0pt}{\lunghbiella}}}
		\pgfpathlineto{\pgfpointadd{\pgfpoint{\pgf@x}{\pgf@y}}{\pgfqpoint{\lunghbiellaa}{0pt}}}
		\disPistone
		\pgfpathlineto{\pgfpointadd{\pgfpoint{\pgf@x}{\pgf@y}}{\pgfqpoint{\lunghbiellaa}{0pt}}}
		\pgfpathlineto{\pgfpointadd{\pgfpoint{\pgf@x}{\pgf@y}}{\pgfqpoint{0pt}{-\lunghbiella}}}
		\pgfpathlineto{\pgfpointadd{\pgfpoint{\pgf@x}{\pgf@y}}{\pgfqpoint{\lunghbiellaa}{0pt}}}
		\disPistone
		\pgfpathlineto{\pgfpointadd{\pgfpoint{\pgf@x}{\pgf@y}}{\pgfqpoint{\lunghbiellaa}{0pt}}}
		\pgfusepath{stroke}
		
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

	}
}

\pgfdeclareshape{gearbox}{
	\inheritsavedanchors[from=rectangle] %
	\inheritanchorborder[from=rectangle]
	\inheritanchor[from=rectangle]{center}
	\inheritanchor[from=rectangle]{north}
	\inheritanchor[from=rectangle]{south}
	\inheritanchor[from=rectangle]{west}
	\inheritanchor[from=rectangle]{east}
	\inheritanchor[from=rectangle]{north west}
	\inheritanchor[from=rectangle]{north east}
	\inheritanchor[from=rectangle]{south east}
	\inheritanchor[from=rectangle]{south west}
	\inheritanchor[from=rectangle]{base}
	%
	
%
%
%
%
%
%
%
	\anchor{center}
	{\pgfpointorigin}
	\foregroundpath{%
		%
		\southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
		\northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
		\pgfpointdiff{\southwest}{\northeast}
		\pgf@xc=\pgf@x		%
		\pgf@yc=\pgf@y		%
		\def\straightw{.1\pgf@xc}
		\def\straighth{.1\pgf@yc}
		
		\pgfpathmoveto{\northeast}
		\pgfpathlineto{\pgfpoint{\pgf@xb}{-\pgf@yb}}
		\pgfpathlineto{\pgfpointadd{\pgfpoint{\pgf@xb}{-\pgf@yb}}{\pgfqpoint{-\straightw}{0pt}}}
		\pgfpathlineto{\pgfpoint{\pgf@xa}{-\straighth}}
		\pgfpathlineto{\pgfpoint{\pgf@xa}{\straighth}}
		\pgfpathlineto{\pgfpointadd{\northeast}{\pgfqpoint{-\straightw}{0pt}}}
		\pgfclosepath
		\pgfusepath{stroke, fill}
	}
}

\makeatother
